Reconstruction of partially sampled multi-band images - Application to STEM-EELS imaging

Electron microscopy has shown to be a very powerful tool to map the chemical nature of samples at various scales down to atomic resolution. However, many samples can not be analyzed with an acceptable signal-to-noise ratio because of the radiation damage induced by the electron beam. This is particularly crucial for electron energy loss spectroscopy (EELS) which acquires spectral-spatial data and requires high beam intensity. Since scanning transmission electron microscopes (STEM) are able to acquire data cubes by scanning the electron probe over the sample and recording a spectrum for each spatial position, it is possible to design the scan pattern and to sample only specific pixels. As a consequence, partial acquisition schemes are now conceivable, provided a reconstruction of the full data cube is conducted as a post-processing step. This paper proposes two reconstruction algorithms for multi-band images acquired by STEM-EELS which exploits the spectral structure and the spatial smoothness of the image. The performance of the proposed schemes is illustrated thanks to experiments conducted on a realistic phantom dataset as well as real EELS spectrum-images.

==> images/S_constraint.tex <==
\begin{tikzpicture}



% \semilogy([qqch xmin xmax log(ymin) log(ymax)])

\newcommand{\semilogx}[5]{
\pgfmathparse{int(#2-1)};\let\Xmax\pgfmathresult
% \draw (0,0) node {#3};
\foreach \ee in{#1,...,\Xmax}{
    \foreach \x in {1,2,3,4,5,6,7,8,9}{
        \draw[thin] ({log10(\x)+\ee},#3) -- ({log10(\x)+\ee},#4);
    };
    \draw[thin, red] (\ee,#3)node[below]{$10^{\ee}$} -- ({\ee},#4);
};
\draw[thin, red] ({#2},#3)node[name=TextX,below]{$10^{#2}$} -- ({#2},#4);

\pgfmathparse{int(#3+#5)}
\let\Valsuivante\pgfmathresult 
\foreach \yy in  {#3,\Valsuivante,...,#4}{
    \draw[thin, red] (#1,\yy) node[left,name=TextY]{$\yy$} -- ({#2},\yy);
};
}

\newcommand{\semilogy}[9]{

\begin{scope}[xshift=#6 +(-#1*#7/(#2-#1))*28.45, yshift=#7 +(-#3*#9/(#4-#3))*28.45 ,xscale=#8/(#2-#1),yscale=#9/(#4-#3)]
\pgfmathparse{int(#4-1)};\let\Ymax\pgfmathresult
% \draw (0,0) node {#3};
\foreach \ee in{#3,...,\Ymax}{
    \foreach \y in {1,2,3,4,5,6,7,8,9}{
        \draw[thin,opacity=0.2] (#1, {log10(\y)+\ee}) -- (#2, {log10(\y)+\ee});
    };
    \draw[thin, red,opacity=0.4] (#1,\ee) -- (#2, {\ee}); % node[left]{$10^{\ee}$}
};
\draw[thin, red,opacity=0.4] (#1,{#4})-- (#2,{#4}); % node[name=TextX,left]{$10^{#4}$} 

\pgfmathparse{int(#1+#5)}
\let\Valsuivante\pgfmathresult 
\foreach \xx in  {#1,\Valsuivante,...,#2}{
    \draw[thin, red,opacity=0.4] (\xx,#3)  -- (\xx,#4); % node[below,name=TextX]{$\xx$}
};
\end{scope}
}









% 10,-5.616065

\begin{scope}[xshift = 10cm, rotate = -90]

\begin{scope}[xscale =6.6174/4, yscale = 6.6174/4 ]

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%





\begin{axis}[%
hide axis,
width=4cm,
height=4cm,
at={(0cm,0cm)},
scale only axis,
xmin=0,
xmax=25,
separate axis lines,
every outer y axis line/.append style={mycolor1},
every y tick label/.append style={font=\color{mycolor1}},
every y tick/.append style={mycolor1},
ymode=log,
ymin=1000,
ymax=10000000,
ytick={       0,  2000000,  4000000,  6000000,  8000000, 10000000},
yminorticks=true,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	8727573.87445925\\
2	2851593.47330894\\
3	118425.165676276\\
4	29279.2968417336\\
5	26194.3404071722\\
6	18651.7766421329\\
7	16204.9910846095\\
8	13059.8164707245\\
9	11249.8995957446\\
10	9955.30855085244\\
11	9078.80230733132\\
12	7946.42234722502\\
13	6932.29444557896\\
14	6219.15146937003\\
15	5409.45270951356\\
16	4796.22082948099\\
17	4311.24090400497\\
18	4039.35739625266\\
19	3673.90196507484\\
20	3326.35061099581\\
21	2806.86717042419\\
22	2433.5774122105\\
};
\end{axis}

\begin{axis}[%
hide axis,
width=4cm,
height=4cm,
at={(0cm,0cm)},
scale only axis,
xmin=0,
xmax=25,
every outer y axis line/.append style={mycolor2},
every y tick label/.append style={font=\color{mycolor2}},
every y tick/.append style={mycolor2},
ymode=log,
ymin=0.0001,
ymax=100,
ytick={  0,  20,  40,  60,  80, 100},
yminorticks=true,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=right
]
\addplot [color=mycolor2, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.0002759473624201\\
2	0.00084504373405419\\
3	0.0207527918664428\\
4	0.0895996397022626\\
5	0.101220062954338\\
6	0.148219234774761\\
7	0.17450412855957\\
8	0.22602865573204\\
9	0.272294571092858\\
10	0.318999363069504\\
11	0.360912132314967\\
12	0.434699668743002\\
13	0.532131551811238\\
14	0.631695864017401\\
15	0.802090004798668\\
16	1.00801845863793\\
17	1.26483735524035\\
18	1.47559581023725\\
19	1.90148268251651\\
20	2.62085654546919\\
21	6.03157255586601\\
22	92.9938475828891\\
};
\end{axis}

\semilogy{0}{25}{-2}{3}{5}{0}{0}{4}{4}

\draw [->,thick] (0,0) -- (4.25,0) node[below] {\Huge b} ;
\draw [->,very thick, mycolor1] (0,0) -- (0,4.5) node[right] {\Huge $\mathbf{\log(\d_b)}$};
\draw [->,very thick, mycolor2] (4,0) -- (4,4.5) node[right] {\Huge $\mathbf{\log(\w_b)}$};

\end{scope}
\end{scope}






% S matrix

\filldraw[fill = red!70,thick] (0,-1) rectangle (10,0); \node at (5,-0.5){\Huge $\S_{1,:}$};
\filldraw[fill = red!50,thick] (0,-2) rectangle (10,-1); \node at (5,-1.5){\Huge $\S_{2,:}$};
\filldraw[fill = red!30,thick] (0,-3) rectangle (10,-2); \node at (5,-2.5){\Huge $\S_{3,:}$};
\filldraw[fill = red!10,thick] (0,-6.616065) rectangle (10,-5.616065); \node at (5,-6.116065){\Huge $\S_{\rhoM,:}$};
\node at (5,-4.3){\Huge $\mathbf{\vdots}$};

\draw[very thick] (0,-6.617403) rectangle (10,0);
\node [anchor = south] at (5,0) {\Huge $\boxed{\S = \H^T\tX}$};


\end{tikzpicture}
